Engineering band selective absorption with epsilon-near-zero media in the infrared

Band-selective absorption and emission of thermal radiation in the infrared are of interest due to applications in emissivity coatings, infrared sensing, thermo-photovoltaics and solar energy harvesting. The broadband nature of thermal radiation presents distinct challenges in achieving spectral and angular selectivity, which are difficult to address by prevalent optical strategies, often yielding restrictive responses. We explore a tri-layer coating employing a nanostructured grating of epsilon-near-zero (ENZ) material, indium tin oxide (ITO), atop a dielectric (silicon dioxide) and metal (gold) underlayer, which shows wide-angle (0-60 degrees) and band-selective (1800 - 2800 nm) high absorption (> 0.8). Numerical simulations and experimental results reveal that the ENZ response of ITO combined with its localized plasmon resonances define the high absorption bandwidth, aided by the sandwiched dielectric's optical properties, elucidating the tunability of the absorption bandwidth. Thermal imaging in the mid-infrared highlights the relevance of the ENZ grating, emphasizing the potential of this coating design as a thermal emitter. This study offers valuable insights into light-matter interactions and opens avenues for practical applications in thermal management and energy harvesting.

==> ref.tex <==
@article{Ding2016,
    author = {Ding, Fei and Dai, Jin and Chen, Yiting and Zhu, Jianfei and Jin, Yi and Bozhevolnyi, Sergey I.},
    journal = {Scientific Reports},
    pages = {1--9},
    title = {{Broadband near-infrared metamaterial absorbers utilizing highly lossy metals}},
    volume = {6},
    year = {2016}
}
@article{Hutley1976,
    author = {Hutley, M. C. and Maystre, D.},
    journal = {Optics Communications},
    number = {3},
    pages = {431--436},
    title = {{The total absorption of light by a diffraction grating}},
    volume = {19},
    year = {1976}
}
@article{Hibbins2006,
    author = {Hibbins, A. P. and Murray, W. A. and Tyler, J. and Wedge, S. and Barnes, W. L. and Sambles, J. R.},
    journal = {Physical Review B - Condensed Matter and Materials Physics},
    number = {7},
    pages = {1--4},
    title = {{Resonant absorption of electromagnetic fields by surface plasmons buried in a multilayered plasmonic nanostructure}},
    volume = {74},
    year = {2006}
}
@article{Carminati2002,
    author = {Greffet and JJ. Carminati, R. , K. and Joulain, Jean-Philippe and Mulet,S. and Mainguy, Y. and Chen},
    journal ={Nature},
    number = {6876},
    pages = {61--64},
    title = {Coherent emission of light by thermal sources},
    volume = {416},
    year = {2002},
}
@article{Landy2008,
    author = {Landy, N. I. and Sajuyigbe, S. and Mock, J. J. and Smith, D. R. and Padilla, W. J.},
    journal = {Physical Review Letters},
    number = {20},
    pages = {1--4},
    title = {{Perfect metamaterial absorber}},
    volume = {100},
    year = {2008},
}
@article{Avitzour2009,
    author = {Avitzour, Yoav and Urzhumov, Yaroslav A. and Shvets, Gennady},
    journal = {Physical Review B - Condensed Matter and Materials Physics},
    number = {4},
    pages = {1--5},
    title = {{Wide-angle infrared absorber based on a negative-index plasmonic metamaterial}},
    volume = {79},
    year = {2009}
}
@article{Liu2011,
    author = {Liu, Xianliang and Tyler, Talmage and Starr, Tatiana and Starr, Anthony F. and Jokerst, Nan Marie and Padilla, Willie J.},
    journal = {Physical Review Letters},
    number = {4},
    pages = {4--7},
    title = {{Taming the blackbody with infrared metamaterials as selective thermal emitters}},
    volume = {107},
    year = {2011}
}
@article{Xu2021,
    author = {Xu, Jin and Raman, Aaswath P.},
    journal = {Science},
    pages = {393--397},
    title = {{Broadband Directional Control of Thermal Emission}},
    volume = {397},
    year = {2021}
}
@article{Sergeant2010,
    author = {Sergeant, Nicholas P. and Agrawal, Mukul and Peumans, Peter},
    journal = {Optics Express},
    number = {6},
    pages = {5525},
    pmid = {20389569},
    title = {{High performance solar-selective absorbers using coated sub-wavelength gratings}},
    volume = {18},
    year = {2010}
}
@article{Ogawa2012,
    author = {Ogawa, Shinpei and Okada, Kazuya and Fukushima, Naoki and Kimata, Masafumi},
    journal = {Applied Physics Letters},
    number = {2},
    title = {{Wavelength selective uncooled infrared sensor by plasmonics}},
    volume = {100},
    year = {2012}
}
@article{Zhang2013,
    author = {Zhang, R. and Zhang, Y. and Dong, Z. C. and Jiang, S. and Zhang, C. and Chen, L. G. and Zhang, L. and Liao, Y. and Aizpurua, J. and Luo, Y. and Yang, J. L. and Hou, J. G.},
    journal = {Nature},
    number = {7452},
    pages = {82--86},
    title = {{Chemical mapping of a single molecule by plasmon-enhanced Raman scattering}},
    volume = {498},
    year = {2013}
}
@article{Cao2009,
    author = {Cao, Linyou and White, Justin S. and Park, Joon Shik and Schuller, Jon A. and Clemens, Bruce M. and Brongersma, Mark L.},
    journal = {Nature Materials},
    number = {8},
    pages = {643--647},
    title = {{Engineering light absorption in semiconductor nanowire devices}},
    volume = {8},
    year = {2009}
}
@article{Anker2008,
    author = {Anker, Jeffrey N and Hall, W Paige and Lyandres, Olga and Shah, Nilam C and Zhao, Jing and Duyne, Richard P Van},
    journal = {Nature Materials},
    pages = {8--10},
    title = { Biosensing with plasmonic nanosensors},
    volume = {7},
    year = {2008}
}
@article{Adato2013,
    author = {Adato, Ronen and Altug, Hatice},
    journal = {Nature Communications},
    title = {{In-situ ultra-sensitive infrared absorption spectroscopy of biomolecule interactions in real time with plasmonic nanoantennas}},
    volume = {4},
    year = {2013}
}
@article{Hirsch2003,
    author = {Hirsch, L. R. and Stafford, R. J. and Bankson, J. A. and Sershen, S. R. and Rivera, B. and Price, R. E. and Hazle, J. D. and Halas, N. J. and West, J. L.},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    number = {23},
    pages = {13549--13554},
    title = {{Nanoshell-mediated near-infrared thermal therapy of tumors under magnetic resonance guidance}},
    volume = {100},
    year = {2003}
}
@article{Raman2014,
    author = {Raman, Aaswath P. and Anoma, Marc Abou and Zhu, Linxiao and Rephaeli, Eden and Fan, Shanhui},
    journal = {Nature},
    number = {7528},
    pages = {540--544},
    title = {{Passive radiative cooling below ambient air temperature under direct sunlight}},
    volume = {515},
    year = {2014}
}
@article{Ni2019,
    author = {Ni, Qing and McBurney, Ryan and Alshehri, Hassan and Wang, Liping},
    journal = {Solar Energy},
    number = {August},
    pages = {623--628},
    title = {{Theoretical analysis of solar thermophotovoltaic energy conversion with selective metafilm and cavity reflector}},
    volume = {191},
    year = {2019}
}
@article{Yang2020,
    author = {Yang, Zhengmei and Ji, Chengang and Cui, Qingyu and Guo, Lingjie Jay},
    journal = {Advanced Optical Materials},
    number = {12},
    pages = {1--10},
    title = {{High-Purity Hybrid Structural Colors by Enhancing Optical Absorption of Organic Dyes in Resonant Cavity}},
    volume = {8},
    year = {2020}
}
@article{Chen2014,
    author = {Chen, Hung Hsin and Hsiao, Hui Hsin and Chang, Hung Chun and Huang, Wei Lun and Lee, Si Chen},
    journal = {Applied Physics Letters},
    number = {8},
    pages = {2--6},
    title = {{Double wavelength infrared emission by localized surface plasmonic thermal emitter}},
    volume = {104},
    year = {2014}
}
@article{Johns2022,
    author = {Johns, Ben and Chattopadhyay, Shashwata and Mitra, Joy},
    journal = {Advanced Photonics Research},
    number = {1},
    pages = {2100153},
    title = {{Tailoring Infrared Absorption and Thermal Emission with Ultrathin Film Interferences in Epsilon‐Near‐Zero Media}},
    volume = {3},
    year = {2022}
}
@article{Rensberg2017,
    author = {Rensberg, Jura and Zhou, You and Richter, Steffen and Wan, Chenghao and Zhang, Shuyan and Sch{\"{o}}ppe, Philipp and Schmidt-Grund, R{\"{u}}diger and Ramanathan, Shriram and Capasso, Federico and Kats, Mikhail A. and Ronning, Carsten},
    journal = {Physical Review Applied},
    number = {1},
    pages = {1--11},
    title = {Epsilon-Near-Zero Substrate Engineering for Ultrathin-Film Perfect Absorbers},
    volume = {8},
    year = {2017}
}
@article{Dey2024,
    author = {Dey, Sraboni and P S, Kirandas and Nagar, Deepshikha Jaiswal and Mitra, Joy},
    title = {Epsilon-Near-Zero Metal Oxide-Based Spectrally Selective Reflectors},
    journal = {ACS Applied Optical Materials},
    volume = {2},
    number = {7},
    pages = {1360-1366},
    year = {2024},
}
@article{Johns2020,
    author = {Johns, Ben and Puthoor, Navas Meleth and Gopalakrishnan, Harikrishnan and Mishra, Akhileshwar and Pant, Ravi and Mitra, J.},
    journal = {Journal of Applied Physics},
    number = {4},
    title = {{Epsilon-near-zero response in indium tin oxide thin films: Octave span tuning and IR plasmonics}},
    volume = {127},
    year = {2020}
}
@article{Vassant2012,
    author = {Vassant, S. and Archambault, A. and Marquier, F. and Pardo, F. and Gennser, U. and Cavanna, A. and Pelouard, J. L. and Greffet, J. J.},
    journal = {Physical Review Letters},
    number = {23},
    pages = {1--5},
    title = {{Epsilon-near-zero mode for active optoelectronic devices}},
    volume = {109},
    year = {2012}
}
@article{Campione2016,
    author = {Campione, Salvatore and Marquier, Francois and Hugonin, Jean Paul and Ellis, A. Robert and Klem, John F. and Sinclair, Michael B. and Luk, Ting S.},
    journal = {Scientific Reports},
    pages = {1--9},
    title = {{Directional and monochromatic thermal emitter from epsilon-near-zero conditions in semiconductor hyperbolic metamaterials}},
    volume = {6},
    year = {2016}
}
@article{Dyachenko2016,
    author = {Dyachenko, P. N. and Molesky, S. and Petrov, A. Yu and St{\"{o}}rmer, M. and Krekeler, T. and Lang, S. and Ritter, M. and Jacob, Z. and Eich, M.},
    journal = {Nature Communications},
    title = {{Controlling thermal emission with refractory epsilon-near-zero metamaterials via topological transitions}},
    volume = {7},
    year = {2016}
}
@article{Shrestha2018,
    author = {Shrestha, Sajan and Wang, Yu and Overvig, Adam C. and Lu, Ming and Stein, Aaron and {Dal Negro}, Luca and Yu, Nanfang},
    journal = {ACS Photonics},
    number = {9},
    pages = {3526--3533},
    title = {{Indium Tin Oxide Broadband Metasurface Absorber}},
    volume = {5},
    year = {2018}
}
@article{Zhou2018,
    author = {Zhou, Kun and Cheng, Qiang and Song, Jinlin and Lu, Lu and Jia, Zhihao and Li, Junwei},
    journal = {Applied Optics},
    number = {1},
    pages = {102},
    pmid = {29328120},
    title = {{Broadband perfect infrared absorption by tuning epsilon-near-zero and epsilon-near-pole resonances of multilayer ITO nanowires}},
    volume = {57},
    year = {2018}
}
@article{Dang2019,
    author = {Dang, Phuc Toan and Le, Khai Q. and Lee, Ji Hoon and Nguyen, Truong Khang},
    journal = {Micromachines},
    number = {10},
    pages = {1--11},
    title = {{A designed broadband absorber based on ENZ mode incorporating plasmonic metasurfaces}},
    volume = {10},
    year = {2019}
}
@article{Osgouei2021,
    author = {Osgouei, Ataollah Kalantari and Hajian, Hodjat and Serebryannikov, Andriy E and Ozbay, Ekmel},
    journal = {Journal of Physics D: Applied Physics},
    number = {27},
    pages = {275102},
    title = {{Hybrid indium tin oxide-Au metamaterial as a multiband bi-functional light absorber in the visible and near-infrared ranges}},
    volume = {54},
    year = {2021}
}
@article{Ji2014,
    author = {Ji, Dengxin and Song, Haomin and Zeng, Xie and Hu, Haifeng and Liu, Kai and Zhang, Nan and Gan, Qiaoqiang},
    journal = {Scientific Reports},
    pages = {1--7},
    title = {{Broadband absorption engineering of hyperbolic metafilm patterns}},
    volume = {4},
    year = {2014}
}
@article{Meng2019,
    author = {Meng, Zhenya and Cao, Hailin and Wu, Xiaodong},
    journal = {Optical Materials},
    pages = {109347},
    title = {{New design strategy for broadband perfect absorber by coupling effects between metamaterial and epsilon-near-zero mode}},
    volume = {96},
    year = {2019}
}
@article{Jiang2022,
    author = {Jiang, Hang and Zhao, Yuanan and Ma, Hao and Feng, Cao and Wu, Yi and Zhang, Weili and Chen, Meiling and Wang, Mengxia and Lian, Yafei and Cao, Zhaoliang and Shao, Jianda},
    journal = {Applied Surface Science},
    title = {{Polarization-Independent, tunable, broadband perfect absorber based on semi-sphere patterned Epsilon-Near-Zero films}},
    volume = {596},
    year = {2022}
}
@book{BracD.B,
    author = {Memoirs and Prévost, Stewart and Kirchhoff, Kirchoff and Bunsen},
    title = {The Laws of Radiation and Absorption},
    publisher = {American Book Company},
    year = {1901},
}
@article{McSherry2022,
    author = {McSherry, Sean and Lenert, Andrej},
    journal = {Applied Physics Letters},
    number = {19},
    pages = {191702},
    title = {{Design of a gradient epsilon-near-zero refractory metamaterial with temperature-insensitive broadband directional emission}},
    volume = {121},
    year = {2022}
}

@article{Gowda2022,
    author = {Gowda, Prarthana and Patient, Dean A. and Horsley, Simon A.R. and Nash, Geoffrey R.},
    journal = {Applied Physics Letters},
    number = {5},
    title = {{Toward efficient and tailorable mid-infrared emitters utilizing multilayer graphene}},
    volume = {120},
    year = {2022}
}
@article{Smith2020,
    author = {Smith, Evan M. and Chen, Jinnan and Hendrickson, Joshua R. and Cleary, Justin W. and Dass, Chandriker and Reed, Amber N. and Vangala, Shivashankar and Guo, Junpeng},
    journal = {Optical Materials Express},
    mendeley-groups = {Emission},
    number = {10},
    pages = {2439},
    title = {{Epsilon-near-zero thin-film metamaterials for wideband near-perfect light absorption}},
    volume = {10},
    year = {2020}
}
@article{Sang2019,
    author = {Sang, Tian and Gao, Jian and Yin, Xin and Qi, Honglong and Wang, La and Jiao, Hongfei},
    journal = {Nanoscale Research Letters},
    publisher = {Nanoscale Research Letters},
    title = {{Angle-Insensitive Broadband Absorption Enhancement of Graphene Using a Multi-Grooved Metasurface}},
    volume = {14},
    year = {2019}
}
@article{TraylorKruschwitz1997,
    author = {{Traylor Kruschwitz}, Jennifer D. and Pawlewicz, Walter T.},
    journal = {Applied Optics},
    number = {10},
    pages = {2157},
    title = {{Optical and durability properties of infrared transmitting thin films}},
    volume = {36},
    year = {1997}
}
@article{Johnson1974,
    author = {Johnson, P. B. and Christy, R. W.},
    journal = {Physical Review B},
    number = {12},
    pages = {5056--5070},
    title = {{Optical constants of transition metals}},
    volume = {9},
    year = {1974}
}























